A Large-Scale Study of Model Integration in ML-Enabled Software Systems

The rise of machine learning (ML) and its integration into software systems has drastically changed development practices. While software engineering traditionally focused on manually created code artifacts with dedicated processes and architectures, ML-enabled systems require additional data-science methods and tools to create ML artifacts -- especially ML models and training data. However, integrating models into systems, and managing the many different artifacts involved, is far from trivial. ML-enabled systems can easily have multiple ML models that interact with each other and with traditional code in intricate ways. Unfortunately, while challenges and practices of building ML-enabled systems have been studied, little is known about the characteristics of real-world ML-enabled systems beyond isolated examples. Improving engineering processes and architectures for ML-enabled systems requires improving the empirical understanding of these systems. We present a large-scale study of 2,928 open-source ML-enabled software systems. We classified and analyzed them to determine system characteristics, model and code reuse practices, and architectural aspects of integrating ML models. Our findings show that these systems still mainly consist of traditional source code, and that ML model reuse through code duplication or pre-trained models is common. We also identified different ML integration patterns and related implementation practices. We hope that our results help improve practices for integrating ML models, bringing data science and software engineering closer together.

==> input/background.tex <==
\section{Motivation and Research Questions}
\label{sec:background}
\noindent\looseness=-1
We present the necessary background, the state of research, as well as motivate and refine our research questions.
%We now provide the required background to motivate our research questions and refine them further.

\looseness=-1
ML-enabled software systems contain ML-based functio-nality, such as prediction, data analysis, or generative content creation\,\cite{feuerriegel2024generative}.
They can incorporate different ML technologies, such as Convolutional Neural Networks (CNNs) for image processing, or Transformers for text generation\,\cite{lecun2015deep,yamashita2018convolutional,vaswani2017attention}.%
%
\label{sec:background:libs}
To implement ML models, ML-enabled systems rely on libraries and frameworks that contain common algorithms and allow developers to build custom ML models. The most popular ones\,\cite{stancin2019libraries} are PyTorch\,\cite{pytorch}, TensorFlow\,\cite{tensorflow}, and Scikit-Learn\,\cite{scilearn}; many others build upon them.
ML models are usually implemented as modular objects building on classes such as ``Module'' (\emph{``BaseEstimator''} in Scikit-Learn). The base class provides a common interface for generic operations used for inference and training networks.

\looseness=-1
\parhead{Characteristics of ML-Enabled Software Systems (\textbf{\textit{RQ1}})}
The integration of ML into software \textit{poses new challenges for development processes, architectures, and testing, among others}\,\cite{bosch2021engineering}.
Many challenges originate from the fundamentally different nature of ML models compared to traditional software\,\cite{nahar2023meta}.
ML models are probabilistic, essentially constituting unreliable functions, while traditional software is more deterministic. While there is extensive theory on the properties of ML in data science, the majority of research and development practices are model-centric. However, integrating ML models into software systems to provide value to end-users requires system-centric engineering methods.
Effective methods need to be tailored towards the actual characteristics and properties of ML in the context of systems.
To this end, we need to improve our empirical understanding of ML-enabled systems in general.
\textit{\textbf{RQ1.1} (What types of systems use ML and how are they related to it?)} first determines what systems\,\cite{idowu2024large,nahar2024product} (e.g., applications or libraries) integrate ML models and how they do it (e.g., do they provide end-user functionality or purely conceptual contributions). This puts the results of our study into context and helps identify differences in the use of ML, and implications for practice.

\looseness=-1
A key difference from traditional software is that ML-enabled systems contain additional artifacts (called \emph{ML assets} in the remainder).
This includes model implementations, model binaries, ML training code, and other ML files\,\cite{idowu2021survey,idowu2022asset,idowu2022emmm}.
These ML assets must be integrated with code and co-evolved. To better understand them, including their relations, \textit{\textbf{RQ1.2} (How much of ML-enabled systems is specific to ML?)} elicits relevant details on the relevance, type, and characteristics of ML assets. %(\challenge{ch2}).} % -- RQ1}

Finally, while quality assurance is an integral part of data science (i.e., validation is part of training), also the integration of the data-centric ML model into the system has to be considered (system-centric view).
However, what are concrete quality assurance practices in ML-enabled systems beyond the validation during the training of ML models themselves has not been captured on a large scale and is limited to individual qualitative studies\,\cite{openja2024empirical}.
To obtain insights on these practices, \textit{\textbf{RQ1.3} (What are quality assurance practices of ML-enabled systems?)} investigates quality assurance on a large scale.

\looseness=-1
\parhead{Reuse of ML Models (\textbf{\textit{RQ2}})}
Similar to reuse in traditional software\,\cite{mojica2013large}, developers reuse ML assets.
However, we lack a full picture of reuse in ML-enabled systems and its specifics.
We know that there is reuse of established ML models, allowing developers to use them without the extensive effort required to build a new model\,\cite{long2022pretrained,qiu2020pretrainednlp}. Such models are called pre-trained models as they are optimized and fully functional.
Pre-trained models for specific tasks are distributed through model hubs\,\cite{jiang2022reusehub}.
While we know sources from which pre-trained models could be reused, we know little about the actual practices, neither how prevalent this reuse is nor how it is realized.
\textit{\textbf{RQ2.1:} (To what extent are pre-trained models used?)} addresses this gap.

Apart from full models, other ML assets (e.g., source code, model binaries) can be reused as well.
However, there are currently no studies on such reuse and its relation to model reuse, e.g., reusing implementations of ML models as an alternative to pre-trained models.
To improve our empirical understanding on the extent and practices behind the reuse of ML assets---addressed by \textit{\textbf{RQ2.2} (To what extent are ML assets reused between ML-enabled systems?)}.

\looseness=-1
\parhead{Architectural Aspects (\textbf{\textit{RQ3}})}
The architecture of ML-enabled systems revolves around ML models, ML assets, and traditional software, which must be integrated together.
This integration poses new challenges as little is known on how the interaction of ML models can impact the behavior of a system.
While some architectures for ML-enabled systems have been proposed, they usually do not focus on concrete interactions and topologies of ML models, but rather on high-level system abstractions.
For instance, a microservice architecture, where ML models are modularized and interact with the rest of the system via REST\,\cite{ribeiro2019microservicearch}.
Others suggest separating ML logic from the business logic of a system\,\cite{yokoyama2019mlarchitecture}.

ML models are typically encapsulated in software modules that contain the ML model (binary) along with source code for model loading and execution, including required pre- and postprocessing steps.
Common anti-patterns include excessive glue code, complicated data-processing pipelines, dead experimental code paths, and lack of abstraction\,\cite{sculley2015}.
Since ML models are updated or replaced regularly\,\cite{Ozkaya2020}, i.e., by an optimized version, which in turn affects the remaining system (e.g., thresholds in glue code need to be adjusted), such anti-patterns hinder optimization.
In contrast, little is known about best practices.
To derive these, \textit{\textbf{RQ3.1} (How are ML models embedded into traditional code?)} investigates current ML model integration patterns.

A case study on Apollo\,\cite{peng2020apollo} showed that systems can contain up to 28 ML models, integrated in complex topologies, with non-trivial interactions and dependencies between models\,\cite{peng2020apollo}.
While current research discusses the implications of such topologies (e.g., propagating error, computational complexity)\,\cite{Peldszus2023, apel2022feature}, it is important to study these in a larger dataset and define common patterns---addressed by \textit{\textbf{RQ3.2} (What are interaction patterns of ML models?)}.





==> input/results.tex <==
\section{Results}
\label{sec:results}


\subsection{Characteristics of ML-enabled Software Systems (\labelcref{it:rq1})}
\label{subsec:rq1}

\subsubsection{Project Type Classification}

In order to characterize the dataset we first conducted a manual classification of the subject systems.

\begin{figure}
	\includegraphics[width=\linewidth]{fig/project_types}
	\caption{Results of the project classification. Projects were classified by type and relation to ML, with one or more labels being assigned in each category.}
	\label{fig:results_classification}
\end{figure}

\subsubsection{Statistics}
\label{subsubsec:results_statistics}

\ys{Use median or average?}

%General statistics
To characterize our subject systems in terms of size we used metrics from GitHub, like the number of stars and commits and additionally counted properties of the code base, like the number of source files, classes and functions and lines of code,. \cref{fig:statistics}.
The median is at 327 stars, 187 commits, 119 source files, ~12,000 lines of code, 113 classes, and 715 functions but there are also outliers with, for example, up to 100,000 stars or 10 million lines of code.\ys{Mention outliers by name?}
The results show that projects span a wide range of sizes, with the majority being of small to medium size. 

\begin{figure}
	\includegraphics[width=\linewidth]{fig/statistics}
	\caption{General statistics of the dataset}
	\label{fig:statistics}
\end{figure}

%ML code
We further measured the quantitative relation between ML-and non-ML code. As shown in \cref{fig:results_ml_files}, the median number of ML-related source files is 42, out of a median of 119 source files, while the median number of ML-related functions is 216 compared to 715 functions in total. This show that around 1/3 of the source code implements ML-related functionality, both on a file level and on a function level.

\begin{figure}
	\includegraphics[width=\linewidth]{fig/results_ml_files}
	\caption{Statistics regarding the share of ML code}
	\label{fig:results_ml_files}
\end{figure}
\begin{figure}
	\includegraphics[width=\linewidth]{fig/results_modules}
	\caption{Number of ML modules implemented in the projects}
	\label{fig:results_models}
\end{figure}

We further investigated the number of artifacts related to ML models. We found that only 339 out of 2,928 repositories (12\%) contain model binary files. Each of these contains a median of 2 such files. Model implementations in source code are much more prevalent, being present in 2,499 repositories. The median number of classes that inherit from "Module" (PyTorch and TensorFlow) or "BaseEstimator" (scikit-learn) is 34. Note that these classes can be either complete models or components of such, so the actual number of ML models is lower. Nevertheless it is safe to assume that the average project contains multiple ML models, since one model is unlikely to be composed of 34 modules.

%Languages
\ys{Relevant?}
In \cref{sec:method} we made the decision to limit our analysis to programs written in Python. Since it is common for software projects to use multiple languages, we analyzed how many source files of other languages are stored in our subject repositories. As shown in \cref{fig:results_lanuage}, the usage of languages other than Python is very limited. Although many projects use additional programming languages, the number of files is relatively low, compared to the number of Python files.

\begin{figure}
	\includegraphics[width=\linewidth]{fig/results_language}
	\caption{Usage of different programming languages}
	\label{fig:results_lanuage}
\end{figure}
%Libraries
Additionally, we investigated the usage of different ML libraries. \Cref{fig:results_library_count} shows that more than half of the projects use more than one ML-library, which constitutes an interesting finding. Concerning the specific libraries we find that PyTorch is the most common, followed by scikit-learn. \ys{I think PyTorch is growing in popularity recently whereas sklearn is becoming less important, but I would need to find sources on that}.
\begin{figure}
	\includegraphics[width=\linewidth]{fig/results_library}
	\caption{Prevalence of different ML libraries and frameworks}
	\label{fig:results_libraries}
\end{figure}
\begin{figure}
	\includegraphics[width=\linewidth]{fig/results_library_number}
	\caption{Number of different ML libraries used within one projects}
	\label{fig:results_library_count}
\end{figure}
\subsubsection{Testing}
\label{subsubsec:results_testing}
\begin{figure}
	\includegraphics[width=\linewidth]{fig/results_tests}
	\caption{Share of functions directly covered by tests for projects that contain at least one unit test}
	\label{fig:results_tests}
\end{figure}

In order to investigate testing practices in our subject systems we analyzed the prevalence of unit tests and the amount of functions directly covered by these tests.
We find that the overall prevalence of unit tests is very low, with only 954 of our subject systems (33\%) containing at least one unit test. The median for those systems is a coverage of only 6\% for all functions and 5.6\% for ML-functions.
We report the portion of functions directly covered by unit tests in \cref{fig:results_tests}, comparing the coverage of ML-related functions to the rest of the codebase. We do not see any major differences here. We also note that the test coverage is generally rather small. This is understandable, considering our results from \cref{it:rq1}.

We further found that 1,091 out of 2,928 repositories (37\%) use continuous integration.
Of these 883 use GitHub actions, 192 use Travis and 16 use Jenkins.

\subsection{Reuse of ML Models (\labelcref{it:rq2})}
\label{subsec:rq2}

\subsubsection{Usage of pre-trained models}

There are 2206 repositories out of a total of 2928 in our dataset that call at least one of the before mentioned APIs that are related to loading ML models. This count includes all APIs, no matter where the model is loaded from. It could include loading a binary that was created from training code in the same system or previously downloaded from a different system. It could also include calls where models are loaded from a remote repository. 1209 of them use an API that is only used to load PTM. 

The average number of API calls per system is ~44.44. The average number of API calls only used to load PTM is ~28.95.
%In average we counted ~3.56 calls that could not be automatically included or omitted as they are not related to an identifier clearly being used for models or data. 

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{fig/results_loadapi_per_system}
	\caption{Number of API calls used to load models.}
	\label{fig:results_all_loads}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{fig/results_modelhub_per_system}
	\caption{Number of API calls used to load models.}
	\label{fig:results_hub_loads}
\end{figure}

We also identified where the models are loaded by looking at the naming of the directories where the models are loaded in. We found that more than half the models which are loaded from a hub are loaded in a directory documented as \textit{test} or \textit{experiment}. 

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{fig/hub_load_where}
\end{figure}
\hk{Would be better if we look at where tests are and if there are loads. Naming of directories is not a good method to do this. [MOVE TO METHODOLOGY]}\\
\hk{TODO: add references, redo labels in graphics, tightlayout for boxplots}\\
\hk{Problems/Results/Discussion on Load Call Analysis:}
\begin{itemize}
	\item \textit{torch.load()} and other API calls are designed so openly that it is difficult to determine weather they acutally load a model
	\item torch: developers usually use multiple load calls to load one model or alternate depending on user input --> multiple loads are flagged for one actual model load and usage
	\item load is not necessarily associated with model usage as initially assumed 
	\item different types of ML require different parts to be loaded (RL: agent, policy; Supervised: Opt, Model, Weights) 
	\item cannot be sure where model is from / identify real ptm
\end{itemize}

\subsection{Reuse of ML-code}
Concerning the code reuse we find the following:
\begin{itemize}
	\item 1,690 out of our 2928 subject systems (~58\%) contain model implementations copied from other systems in the dataset
	\item These projects copied an average of 18 files related to the implementation of ML models out of an average of 34 files, leading to a copy rate of 53\%
	\item We find that among the duplicates there are 405 clusters, with most clusters containing less than 10 systems \ys{TODO: Update once new results are available}
	\item There are some larger clusters, as shown in \cref{tab:clusters}.
\end{itemize}

\begin{table}
	\centering
	\caption{Overview of the 10 largest clusters of duplicated projects.\ys{TODO: Update once new results are available}}
	\label{tab:clusters}
	\begin{tabular}{r|l}
		\textbf{Cluster size} & \textbf{Original Project} \\
		\hline
		257 & open-mmlab/mmdetection \\
		249 & facebookresearch/fairseq \\
		149 & huggingface/transformers \\
		56 & open-mmlab/OpenPCDet\\
		44 & CompVis/stable-diffusion\\
		39 & OpenNMT/OpenNMT-py\\
		30 & open-mmlab/mmdetection3d \\
		29 & locuslab/convmixer \\
		28 & open-mmlab/mmsegmentation
	\end{tabular}
	
\end{table}


\subsection{Architecture of ML-Enabled Software Systems (\labelcref{it:rq3})}
\label{subsec:rq3}
\ys{Notes and todos}

\begin{table*}
\scriptsize
	\caption{Summary of the systems analyzed}
	\begin{tabularx}{\textwidth}{llXXXXXXXX}
		ID & Name                               & Task                                          & Storage       & Training    & Input               & Output                     & Number & Interaction             & Type                                 \\ \hline
		0  & duongcongnha/Vehicle-tracking      & Object tracking                               & Local, remote & Pretrained  & Images              & Bounding Boxes             & 2      & Sequential              & CNN                                  \\
		1  & jonaswinkler/paperless-ng          & Assign labels to text                         & Local         & Custom      & Text                & Labels                     & 3      & Parallel                & MLP                                  \\
		2  & pixelite1201/BEDLAM                & Pose estimation                               & None          & Fine-tuned  & Images              & Dictionary of numeric data & 2      & Alternative             & CNN                                  \\
		3  & chrisdonahue/sheetsage             & Transcribe music                              & Remote        & Unknown     & Audio               & Text                       & 2      & Parallel                & Transformer                          \\
		4  & sunnyhaibin/sunnypilot             & E2E Autonomous Driving                        & Remote        & Pre-trained & Images              & Actions                    & 2      & Parallel                & Unkown                               \\
		5  & husseinmozannar/SOQAL              & Chatbot                                       & Remote        & Fine-tuned  & Unkown              & Unkown                     & 1      &                         & Transformer                          \\
		6  & pysal/spopt                        & Optimization for spatial data                 & Local         & Custom      & Geopandas-Dataframe & Clusters                   & 2      & Parallel                & Clustering                           \\
		7  & HW140701/VideoTo3dPoseAndBvh       & Pose estimation                               & Local         & Pre-trained & Video               & BVH/mp4                    & 4      & Sequential, Alternative & CNN                                  \\
		8  & mbzuai-oryx/Video-ChatGPT          & Chatbot, video processing                     & Remote, local & Pre-trained & Video + Text        & Text                       & 2      & Sequential              & LLM                                  \\
		9  & Zhongdao/UniTrack                  & Object Tracking/ Segmentation/ Classification & Remote        & Pre-trained & Images              & Bounding boxes             & 2      & Alternative             & CNN                                  \\
		10 & PhonologicalCorpusTools/CorpusTool & Visualizing data                              & Local         & Custom      & Unkown              & Unkown                     & 1      &                         & PCA                                  \\
		11 & Pinafore/qb                        & Chatbot                                       & Remote        & Pre-trained & Text                & Text                       & 3      & Alternative             & Unkown                               \\
		12 & JaidedAI/EasyOCR                   & Optical character recognition                 & Remote        & Pre-trained & Images              & Text                       & 4      & Sequential, alternative & CNN, RNN                             \\
		13 & facebookresearch/sound-spaces      & Navigation                                    & Local         & Custom      & Images, Sound       & Actions | Waypoints        & 10     & Fusion, alternative     & CNN, RNN, Transformer                \\
		14 & reqtrade/freqtrade                 & Cryptotrading                                 & Local         & Custom      & Unknown             & Unkown                     & 18     & Alternative             & Gradien Boosting, Random Forest, MLP
	\end{tabularx}
\end{table*}

